Cross-modal codification of images with auditory stimuli: a language for the visually impaired

In this study we describe a methodology to realize visual images cognition in the broader sense, by a cross-modal stimulation through the auditory channel. An original algorithm of conversion from bi-dimensional images to sounds has been established and tested on several subjects. Our results show that subjects where able to discriminate with a precision of 95\% different sounds corresponding to different test geometric shapes. Moreover, after brief learning sessions on simple images, subjects where able to recognize among a group of 16 complex and never-trained images a single target by hearing its acoustical counterpart. Rate of recognition was found to depend on image characteristics, in 90% of the cases, subjects did better than choosing at random. This study contribute to the understanding of cross-modal perception and help for the realization of systems that use acoustical signals to help visually impaired persons to recognize objects and improve navigation

==> references_ksh <==
@comment{x-kbibtex-personnameformatting=<%l><, %f>}

@article{russ2010,
	abstract = "{Russell TL, Werblin FS. Retinal synaptic pathways underlying the response of the rabbit local edge detector. J Neurophysiol 103: 2757-2769, 2010. First published March 24, 2010; doi:10.1152/jn.00987.2009. We studied the circuitry that underlies the behavior of the local edge detector (LED) retinal ganglion cell in rabbit by measuring the spatial and temporal properties of excitatory and inhibitory currents under whole cell voltage clamp. Previous work showed that LED excitation is suppressed by activity in the surround. However, the contributions of outer and inner retina to this characteristic and the neurotransmitters used are currently unknown. Blockage of retinal inhibitory pathways (GABA(A), GABA(C), and glycine) eliminated edge selectivity. Inverting gratings in the surround with 50-mu m stripe sizes did not stimulate horizontal cells, but suppressed ON and OFF excitation by roughly 60\%, indicating inhibition of bipolar terminals (feedback inhibition). On pharmacologic blockage, we showed that feedback inhibition used both GABA(A) and GABA(C) receptors, but not glycine. Glycinergic inhibition suppressed GABAergic feedback inhibition in the center, enabling larger excitatory currents in response to luminance changes. Excitation, feedback inhibition, and direct (feedforward) inhibition responded to luminance-neutral flipping gratings of 20- to 50-mu m widths, showing they are driven by independent subunits within their receptive fields, which confers sensitivity to borders between areas of texture and nontexture. Feedforward inhibition was glycinergic, its rise time was faster than decay time, and did not function to delay spiking at the onset of a stimulus. Both the ON and OFF phases could be triggered by luminance shifts as short in duration as 33 ms and could be triggered during scenes that already produced a high baseline level of feedforward inhibition. Our results show how LED circuitry can use subreceptive field sensitivity to detect visual edges via the interaction between excitation and feedback inhibition and also respond to rapid luminance shifts within a rapidly changing scene by producing feedforward inhibition.}",
	address = "{9650 ROCKVILLE PIKE, BETHESDA, MD 20814 USA}",
	affiliation = "{Werblin, FS (Reprint Author), Univ Calif Berkeley, Dept Mol \& Cell Biol, Div Neurobiol, 145 LSA, Berkeley, CA 94720 USA. Russell, Thomas L.; Werblin, Frank S., Univ Calif Berkeley, Dept Mol \& Cell Biol, Div Neurobiol, Berkeley, CA 94720 USA.}",
	author = "Russell, Thomas L. and Werblin, Frank S.",
	author-email = "{werblin@berkeley.edu}",
	doc-delivery-number = "{594UN}",
	doi = "10.1152/jn.00987.2009",
	funding-acknowledgement = "{National Eye Institute {[}EY-015512]}",
	funding-text = "{This work was supported by National Eye Institute Grant EY-015512.}",
	issn = "{0022-3077}",
	journal = "{Journal of Neurophysiology}",
	journal-iso = "{J. Neurophysiol.}",
	keywords-plus = "{PARASOL GANGLION-CELLS; BIPOLAR CELLS; RECEPTIVE-FIELD; HORIZONTAL CELLS; DISRUPTIVE COLORATION; FUNCTIONAL CIRCUITRY; LATERAL INTERACTIONS; CONE PHOTORECEPTORS; MAMMALIAN RETINA; INHIBITION}",
	language = "{English}",
	month = "{MAY}",
	number = "{5}",
	number-of-cited-references = "{50}",
	pages = "{2757--2769}",
	publisher = "{AMER PHYSIOLOGICAL SOC}",
	research-areas = "{Neurosciences \& Neurology; Physiology}",
	times-cited = "{15}",
	title = "{Retinal Synaptic Pathways Underlying the Response of the Rabbit Local Edge Detector}",
	type = "{Article}",
	unique-id = "{ISI:000277564500040}",
	volume = "{103}",
	web-of-science-categories = "{Neurosciences; Physiology}",
	year = "{2010}"
}

@article{pasu1999,
	abstract = "{Responses to contour features in macaque area V4. J. Neurophysiol. 82: 2490-2502, 1999. The ventral pathway in visual cortex is responsible for the perception of shape. Area V4 is an important intermediate stage in this pathway, and provides the major input to the final stages in inferotemporal cortex. The role of V4 in processing shape information is not yet clear. We studied V4 responses to contour features (angles and curves), which many theorists have proposed as intermediate shape primitives. We used a large parametric set of contour features to test the responses of 152 V4 cells in two awake macaque monkeys. Most cells responded better to contour features than to edges or bars, and about one-third exhibited systematic tuning for contour features. In particular, many cells were selective for contour feature orientation, responding to angles and curves pointing in a particular direction. There was a strong bias toward convex (as opposed to concave) features, implying a neural basis for the well-known perceptual dominance of convexity. Our results suggest that V4 processes information about contour features as a step toward complex shape recognition.}",
	address = "{9650 ROCKVILLE PIKE, BETHESDA, MD 20814 USA}",
	affiliation = "{Connor, CE (Reprint Author), Johns Hopkins Univ, Zanvyl Krieger Mind Brain Inst, 338 Krieger Hall,3400 N Charles St, Baltimore, MD 21218 USA. Johns Hopkins Univ, Zanvyl Krieger Mind Brain Inst, Baltimore, MD 21218 USA. Johns Hopkins Univ, Dept Biomed Engn, Baltimore, MD 21218 USA. Johns Hopkins Univ, Dept Neurosci, Baltimore, MD 21218 USA.}",
	author = "Pasupathy, A and Connor, CE",
	doc-delivery-number = "{259CE}",
	issn = "{0022-3077}",
	journal = "{JOURNAL OF NEUROPHYSIOLOGY}",
	journal-iso = "{J. Neurophysiol.}",
	keywords-plus = "{INFEROTEMPORAL CORTEX; OBJECT RECOGNITION; CARTESIAN GRATINGS; SHAPE-RECOGNITION; VISUAL PROPERTIES; NEURONS; MONKEY; FORM; CURVATURE; PARTS}",
	language = "{English}",
	month = "{NOV}",
	number = "{5}",
	number-of-cited-references = "{51}",
	pages = "{2490--2502}",
	publisher = "{AMER PHYSIOLOGICAL SOC}",
	research-areas = "{Neurosciences \& Neurology; Physiology}",
	times-cited = "{247}",
	title = "{Responses to contour features in macaque area V4}",
	type = "{Article}",
	unique-id = "{ISI:000083875700041}",
	volume = "{82}",
	web-of-science-categories = "{Neurosciences; Physiology}",
	year = "{1999}"
}

@article{henr1994,
	address = "{THE BOULEVARD, LANGFORD LANE, KIDLINGTON, OXFORD, ENGLAND OX5 1GB}",
	affiliation = "{HENRY, GH (Reprint Author), AUSTRALIAN NATL UNIV,JOHN CURTIN SCH MED RES,DIV NEUROSCI,CTR VISUAL SCI,GPO BOX 334,CANBERRA,ACT 2601,AUSTRALIA. VANDERBILT UNIV,DEPT PSYCHOL,NASHVILLE,TN 37240.}",
	author = "Henry, GH and Michalski, A and Winborne, BM and McCart, RJ",
	doc-delivery-number = "{PH714}",
	doi = "10.1016/0301-0082(94)90061-2",
	issn = "{0301-0082}",
	journal = "{Progress in Neurobiology}",
	journal-iso = "{Prog. Neurobiol.}",
	keywords-plus = "{CAT STRIATE CORTEX; RECEPTIVE-FIELD PROPERTIES; MONKEY SUPERIOR COLLICULUS; LATERAL GENICULATE-NUCLEUS; BASIC NETWORK PRINCIPLES; RETINAL GANGLION-CELLS; CROSS-CORRELATION ANALYSIS; DARK-REARED KITTENS; CORTICAL-CELLS; RESPONSE PROPERTIES}",
	language = "{English}",
	month = "{Jul-Aug}",
	number = "{4-5}",
	number-of-cited-references = "{321}",
	pages = "{381--437}",
	publisher = "{PERGAMON-ELSEVIER SCIENCE LTD}",
	research-areas = "{Neurosciences \& Neurology}",
	times-cited = "{26}",
	title = "{The nature and origin of orientation specificity in neurons of the visual pathways}",
	type = "{Review}",
	unique-id = "{ISI:A1994PH71400003}",
	volume = "{43}",
	web-of-science-categories = "{Neurosciences}",
	year = "{1994}"
}

@conference{Yukio2004,
	author = "Yukio, S. and Takeo, K. and Kazukiyo, Y. and Kimiyasu, S.",
	booktitle = "{OCEANS '04. MTTS/IEEE TECHNO-OCEAN '04}",
	doi = "10.1109/OCEANS.2004.1406390",
	pages = "1759--1764",
	publisher = "IEEE",
	title = "{Basic study on the sign for the visually impaired person in a beach institution}",
	volume = "3",
	year = "2004"
}

@proceedings{proceedings,
	address = "The address of the publisher",
	editor = "Kidwelly, Peter",
	month = 7,
	note = "An optional note",
	organization = "The organization",
	publisher = "The name of the publisher",
	series = 5,
	title = "{The title of the work}",
	volume = 4,
	year = 1993
}

@book{book,
	address = "The address",
	author = "Babington, Peter",
	edition = 3,
	isbn = "3257227892",
	month = 7,
	note = "An optional note",
	publisher = "The name of the publisher",
	series = 10,
	title = "{The title of the work}",
	volume = 4,
	year = 1993
}

@conference{kish2013,
	//organization = "",
	address = "PO BOX 211, 1000 AE Amsterdam, Netherlands",
	author = "{Kishino, T and Zhe, S and Micheletto, R}",
	booktitle = "{New Trends in Image Analysis and Processing -- ICIAP 2013}",
	doi = "10.1016/S0262-8856(97)00087-5",
	editor = "Petrosino, A and Maddalena, L and Pala, P",
	issn = "{0262-8856}",
	month = "Apr 3",
	pages = "251--263",
	publisher = "Elsevier Science BV",
	series = 4,
	title = "{A Fast and Precise HOG-Adaboost Based Visual Support System Capable to Recognize Pedestrian and Estimate Their Distance}",
	volume = 16,
	year = 2013
}

@article{nnnn,
	abstract = "{This paper describes a portable vision-based obstacle detection system, intended for use by blind people. The system combines an obstacle detection system designed for AGVs with recalibration of ground position and a Kalman Filter based model of the person's walking movement. The system uses stereo vision. Obstacle detection is achieved through comparison of the disparity seen with that expected from the position of the ground. Recalibration of ground position is made by plane fitting in the ground region. Motion estimation using two visual methods and the use of an inclinometer is described. The results show satisfactory success in all parts of the system. (C) 1998 Elsevier Science B.V.}",
	address = "{PO BOX 211, 1000 AE AMSTERDAM, NETHERLANDS}",
	affiliation = "{Molton, N (Reprint Author), Univ Oxford, Dept Engn Sci, Parks Rd, Oxford OX1 3PJ, England. Univ Oxford, Dept Engn Sci, Oxford OX1 3PJ, England.}",
	author = "Kishino, T and Zhe, S and Micheletto, R",
	doc-delivery-number = "{ZF885}",
	doi = "10.1016/S0262-8856(97)00087-5",
	issn = "{0262-8856}",
	journal = "{New Trends in Image Analysis and Processing -- ICIAP 2013}",
	journal-iso = "{Image Vis. Comput.}",
	keywords = "{obstacle avoidance; mobility aids; visual navigation}",
	keywords-plus = "{MOTION}",
	language = "{English}",
	month = "{APR 3}",
	number = "{4}",
	number-of-cited-references = "{23}",
	pages = "{251--263}",
	publisher = "{ELSEVIER SCIENCE BV}",
	research-areas = "{Computer Science; Engineering; Optics}",
	times-cited = "{33}",
	title = "{A Fast and Precise HOG-Adaboost Based Visual Support System Capable to Recognize Pedestrian and Estimate Their Distance}",
	type = "{Article}",
	unique-id = "{ISI:000072943000004}",
	volume = "{16}",
	web-of-science-categories = "{Computer Science, Artificial Intelligence; Computer Science, Software Engineering; Computer Science, Theory \& Methods; Engineering, Electrical \& Electronic; Optics}",
	year = "{2013}"
}

@article{molt1998,
	abstract = "{This paper describes a portable vision-based obstacle detection system, intended for use by blind people. The system combines an obstacle detection system designed for AGVs with recalibration of ground position and a Kalman Filter based model of the person's walking movement. The system uses stereo vision. Obstacle detection is achieved through comparison of the disparity seen with that expected from the position of the ground. Recalibration of ground position is made by plane fitting in the ground region. Motion estimation using two visual methods and the use of an inclinometer is described. The results show satisfactory success in all parts of the system. (C) 1998 Elsevier Science B.V.}",
	address = "{PO BOX 211, 1000 AE AMSTERDAM, NETHERLANDS}",
	affiliation = "{Molton, N (Reprint Author), Univ Oxford, Dept Engn Sci, Parks Rd, Oxford OX1 3PJ, England. Univ Oxford, Dept Engn Sci, Oxford OX1 3PJ, England.}",
	author = "Molton, N and Se, S and Brady, JM and Lee, D and Probert, P",
	doc-delivery-number = "{ZF885}",
	doi = "10.1016/S0262-8856(97)00087-5",
	issn = "{0262-8856}",
	journal = "{IMAGE AND VISION COMPUTING}",
	journal-iso = "{Image Vis. Comput.}",
	keywords = "{obstacle avoidance; mobility aids; visual navigation}",
	keywords-plus = "{MOTION}",
	language = "{English}",
	month = "{APR 3}",
	number = "{4}",
	number-of-cited-references = "{23}",
	pages = "{251--263}",
	publisher = "{ELSEVIER SCIENCE BV}",
	research-areas = "{Computer Science; Engineering; Optics}",
	times-cited = "{33}",
	title = "{A stereo vision-based aid for the visually impaired}",
	type = "{Article}",
	unique-id = "{ISI:000072943000004}",
	volume = "{16}",
	web-of-science-categories = "{Computer Science, Artificial Intelligence; Computer Science, Software Engineering; Computer Science, Theory \& Methods; Engineering, Electrical \& Electronic; Optics}",
	year = "{1998}"
}

@article{snai1998,
	abstract = "{Established mobility aids, such as the long cane, enable visually impaired users to travel safely in urban environments. This paper describes continuing work to enhance this mobility by providing a series of high-level navigational goals. In particular, we describe algorithms to detect doorways and to facilitate centre-path travel. To maintain high performance at low cost, both algorithms use sparsely-sampled images from a single camera. Doorway detection is achieved by the detection of characteristic patterns of near-vertical and near-horizontal lines. The direction of travel along a path is determined by locating the dominant vanishing point of the lines in the image. Experimental results are presented for both algorithms. (C) 1998 Elsevier Science B.V.}",
	address = "{PO BOX 211, 1000 AE AMSTERDAM, NETHERLANDS}",
	affiliation = "{Lee, D (Reprint Author), Univ Oxford, Dept Engn Sci, Robot Res Grp, Parks Rd, Oxford OX1 3PJ, England. Univ Oxford, Dept Engn Sci, Robot Res Grp, Oxford OX1 3PJ, England.}",
	author = "Snaith, M and Lee, D and Probert, P",
	doc-delivery-number = "{ZF885}",
	doi = "10.1016/S0262-8856(97)00094-2",
	issn = "{0262-8856}",
	journal = "{IMAGE AND VISION COMPUTING}",
	journal-iso = "{Image Vis. Comput.}",
	keywords = "{visual impairment; feature detection; navigation}",
	language = "{English}",
	month = "{APR 3}",
	number = "{4}",
	number-of-cited-references = "{14}",
	pages = "{225--233}",
	publisher = "{ELSEVIER SCIENCE BV}",
	research-areas = "{Computer Science; Engineering; Optics}",
	times-cited = "{10}",
	title = "{A low-cost system using sparse vision for navigation in the urban environment}",
	type = "{Article}",
	unique-id = "{ISI:000072943000002}",
	volume = "{16}",
	web-of-science-categories = "{Computer Science, Artificial Intelligence; Computer Science, Software Engineering; Computer Science, Theory \& Methods; Engineering, Electrical \& Electronic; Optics}",
	year = "{1998}"
}

@article{kubo2001,
	author = "Kubovy, Michael and Valkenburg, David Van",
	journal = "Cognition",
	pages = "97--126",
	title = "{Auditory and visual objects}",
	volume = "80",
	year = "2001"
}

@article{arno2005,
	author = "{Derek H. Arnold}, Alan Johnston and Nishida, Shinya",
	journal = "Vision Research",
	pages = "1275--1284",
	title = "{Timing sight and sound}",
	volume = "45",
	year = "2005"
}

@article{tura2005,
	author = "{Massimo Turatto}, Veronica Mazza and Umilta, Carlo",
	journal = "Cognition",
	pages = "B55--B64",
	title = "{Crossmodal object-based attention: Auditory objects affect visual processing}",
	volume = "96",
	year = "2005"
}

@article{sham2010,
	author = "Shams, Ladan and Kim, Robyn",
	journal = "Physics of Life reviews",
	pages = "269--284",
	title = "{Crossmodal influences on visual perception}",
	volume = "7",
	year = "2010"
}

@article{ziem2013,
	author = "{Michal Ziembowicz}, Andrzej Nowak and Winkielman, Piotr",
	journal = "Cognition",
	pages = "273--278",
	title = "{When sounds look right and images sound correct: Cross-modal coherence enhances claims of pattern presence}",
	volume = "129",
	year = "2013"
}

@article{buck2010,
	author = "{David Buckley}, Charlotte Codina Palvi Bhardwaj and Pascalis, Olivier",
	journal = "Vision Research",
	pages = "548--556",
	title = "{Action video game players and deaf observers have larger Goldmann visual fields}",
	volume = "50",
	year = "2010"
}

@article{bomb2010,
	author = "Bomba, Marie D. and Singhal, Anthony",
	journal = "Brain and Cognition",
	pages = "273--280",
	title = "{ERP evidence of early cross-modal links between auditory selective attention and visuo-spatial memory}",
	volume = "74",
	year = "2010"
}

@article{Yoshihiro1996,
	author = "Kawai, Yoshihiro and Tomita, Fumiaki",
	journal = "Journal of the Institute of Image Information and Television Engineers",
	pages = "325--328",
	title = "{A Support System for the Visually Disabled to Recognized 3D Objects}",
	volume = "51",
	year = "1996"
}

@article{kobayashi1997,
	author = "Kobayashi, Makoto and Ohta, Michio",
	journal = "Society of Biomechanisms (SOBIM) Japan",
	number = "1",
	pages = "39--42",
	title = "{Sound Localization Using Image Information for an Acoustic Visual Aid System}",
	volume = "21",
	year = "1997"
}

@article{Lew2004,
	author = "Lewald, Jorg and Guski, Rainer",
	doi = "10.1016/j.neulet.2003.12.045",
	journal = "Neuroscience Letters",
	number = "",
	pages = "119--122",
	title = "{Auditory-visual temporal integration as a function of distance: no compensation for sound-transmission time in human perception}",
	volume = "357",
	year = "2004"
}

@article{Nakamura1997,
	author = "Nakamura, Kazuhiro and Aono, Yoshiyuki and Tadokoro, Yoshiaki",
	journal = "Systems and Computers in Japan",
	number = "13",
	pages = "36--45",
	title = "{A Walking Navigation System for the Blind}",
	volume = "28",
	year = "1997"
}

@article{Kaluwahandi2001,
	author = "Sasadara, Kaluwahandi and Yoshiaki, Tadokoro",
	journal = "Journal of the Institute of Image Information and Television Engineers",
	number = "11",
	pages = "1499--1505",
	title = "{Study of a Portable Traveling Support System using Image Processing for the Visually Impaired}",
	volume = "55",
	year = "2001"
}

@article{suzuki2003,
	author = "Yuji, Suzuki and Hiroyasu, Hiraiwa and Yoshinori, Takeuchi and Tetsuya, Matsumoto and Hiroaki, Kudoh and Noboru, Ohnishi",
	journal = "IEEJ Transactions on Electronics, Information and Systems",
	number = "738",
	pages = "13--18",
	title = "{A System for Extracting Character Information in the Environment for Visually Impaired People}",
	volume = "102",
	year = "2003"
}

@article{tanaka2008,
	author = "Makoto, Tanaka and Hideaki, Goto",
	journal = "Information Processing Society of Japan :Computer Vision and Image Media",
	pages = "125--130",
	title = "{Wearable Reading Assistant Device for the Blind}",
	volume = "115",
	year = "2008"
}

@article{Watanabe2000,
	author = "{Watanabe Tetsuya}, Kume Yuichiro and Tohru, Ifukube",
	journal = "Journal of the Institute of Image Information and Television Engineers",
	number = "6",
	pages = "840--847",
	title = "{Shape Discrimination with a Tactile Mouse}",
	volume = "54",
	year = "2000"
}

@article{Watanabe20002,
	author = "Tetsuya, Watanabe and Makoto, Kobayashi",
	journal = "IEICE Technical Report Japan",
	number = "112",
	pages = "27--32",
	title = "{Development of an electronic raise-writer for transmitting graphical information among blind people}",
	volume = "100",
	year = "2000"
}

@article{John2000,
	author = "{John J. McDonald}, Wolfgang A. Teder-S{\"a}lej{\"a}rvi and Hillyard, Steven A.",
	journal = "Nature",
	number = "6806",
	pages = "906--908",
	title = "{Involuntary orienting to sound improves visual perception}",
	volume = "407",
	year = "2000"
}

@article{Holroyd2002,
	author = "B., Holroyd Clay and G.H., Coles Michael",
	journal = "Psychological Review",
	number = "4",
	pages = "679--709",
	title = "{The neural basis of human error processing: Reinforcement learning, dopamine, and the error-related negativity.}",
	volume = "109",
	year = "2002"
}

@article{Shiffrin1977,
	author = "M., Shiffrin Richard and Walter, Schneider",
	journal = "Psychological Review",
	number = "2",
	pages = "127--190",
	title = "{Controlled and automatic human information processing: II. Perceptual learning, automatic attending and a general theory.}",
	volume = "84",
	year = "1977"
}

@article{Meijer1992,
	author = "Meijer, P.B.L.",
	issn = "0018-9294",
	journal = "Biomedical Engineering, IEEE Transactions on",
	number = "2",
	pages = "112--121",
	title = "{An experimental system for auditory image representations}",
	volume = "39",
	year = "1992"
}


